Privacy-Preserving and Trustworthy Deep Learning for Medical Imaging

The shift towards efficient and automated data analysis through Machine Learning (ML) has notably impacted healthcare systems, particularly Radiomics. Radiomics leverages ML to analyze medical images accurately and efficiently for precision medicine. Current methods rely on Deep Learning (DL) to improve performance and accuracy (Deep Radiomics). Given the sensitivity of medical images, ensuring privacy throughout the Deep Radiomics pipeline-from data generation and collection to model training and inference-is essential, especially when outsourced. Thus, Privacy-Enhancing Technologies (PETs) are crucial tools for Deep Radiomics. Previous studies and systematization efforts have either broadly overviewed PETs and their applications or mainly focused on subsets of PETs for ML algorithms. In Deep Radiomics, where efficiency, accuracy, and privacy are crucial, many PETs, while theoretically applicable, may not be practical without specialized optimizations or hybrid designs. Additionally, not all DL models are suitable for Radiomics. Consequently, there is a need for specialized studies that investigate and systematize the effective and practical integration of PETs into the Deep Radiomics pipeline. This work addresses this research gap by (1) classifying existing PETs, presenting practical hybrid PETS constructions, and a taxonomy illustrating their potential integration with the Deep Radiomics pipeline, with comparative analyses detailing assumptions, architectural suitability, and security, (2) Offering technical insights, describing potential challenges and means of combining PETs into the Deep Radiomics pipeline, including integration strategies, subtilities, and potential challenges, (3) Proposing potential research directions, identifying challenges, and suggesting solutions to enhance the PETs in Deep Radiomics.

==> backup.tex <==

Previous studies have extensively reviewed PETs and their intersections with ML, with a typical focus either solely on PETs, considering their diverse applications, or specifically on existing ML schemes as part of literature reviews. However, our research emphasizes developing privacy-preserving solutions for the emerging field of Deep Radiomics within precision medicine. Thus, identifying potential solutions and associated challenges throughout the pipeline is crucial. Although all PETs may theoretically apply to Deep Radiomics, their performance limitations stemming from theoretical constructs may impede their practicality, necessitating either their ignorance or a hybrid approach. Therefore, devising a roadmap for effectively integrating such solutions into Deep Radiomics is essential but missing in the literature. Studies in the literature that have explored multiple PETs can be summarized accordingly: Studies \cite{darzi2024pqcmeetsml,ppmlpqc} explored PETs in the post-quantum era, while \cite{ppmlcheng,Xu2021PrivacyPreservingML,SokPPML,ppmlacmsurvey} primarily discuss PPML from the perspective of ML. Additionally, \cite{smartppmlnpsmart} examines encrypted computation, with \cite{ng2023sok,qin2023cryptographic} providing in-depth analyses, and \cite{ppdlsurvtanuwidjaja2020privacy} showcases their hybridization with other PETs such as DP. Furthermore, \cite{ppdlcabrero2021sok} illustrates their integration with TEEs. Studies like \cite{ppdlsurvboulemtafes2020review,ppdlmireshghallah2020privacy} classify existing works in the phases of learning, inference, and model release, discussing the roles of Multi-Party Computation (MPC), Homomorphic Encryption (HE), and DP in these phases. However, \cite{ppdlantwi2021privacy} only categorizes Collaborative Deep Learning under the training stage. Despite numerous works in the literature focusing on PETs and their broad applications or discussing their integration with ML, there appears to be a gap in the literature concerning how these PETs can specifically benefit ML in a particular application.




\section{Introduction}\label{sec:introduction}
\IEEEPARstart{A}{s} traditional technologies are progressively replaced by digital alternatives, and there has been a substantial increase in digital data generation, highlighting the Big Data trend. This trend is especially noticeable in the medical sector, where clinical routine information (e.g., medical images \cite{}) is increasingly being digitized, resulting in the creation of Electronic Health Records (EHRs) \cite{huang2020fusion}. In medicine, diverse methods for generating extensive data are prevalent, such as genomics \cite{jiang2022big} and proteomics \cite{cui2022high}. Additionally, with the growing adoption of imaging modalities, the National Institutes of Health (NIH) has highlighted Radiomics \cite{jha2023emerging} as a promising technique for quantitatively analyzing high-dimensional medical imaging data, with applications extending beyond MRI to include modalities like ultrasound, computed tomography (CT), and nuclear medicine imaging.

With the increased volume of data generated for Radiomics (images), storage has become a significant concern. Cloud storage services have gained traction as a promising solution because they provide vast and cost-effective storage solutions accessible from anywhere. However, EHRs contain sensitive patient information, making storing such data on remote Cloud servers, even if the server is trusted (e.g., a known company), highly inadvisable. To preserve the confidentiality of outsourced data, cryptographic tools (e.g., encryption) can be utilized to encrypt data before storing it on the Cloud. However, medical records are frequently read (search) and updated (e.g., a hospital accessing patients' records), necessitating efficient search and update operations. Regular encryption methods (e.g., using AES) provide confidentiality but do not support these operations efficiently, as they require downloading the entire encrypted dataset for decryption, leading to substantial communication overhead. Hence, it is crucial to use alternative methods that provide data privacy, efficient search, and update operations on outsourced encrypted data.

While secure storage of extensive Radiomics data can be addressed, traditional methods for processing this data, such as a hospital examining CT images for statistical studies, are time-consuming, error-prone, and potentially inaccurate. Integrating Machine learning into various applications has emerged as a promising solution for extracting structural knowledge from datasets, enabling precise outcome predictions. For instance, Deep Learning (DL) has proven effective in Radiomics \cite{fromMLtoDeep,TraditionalMLtoCNN,gupta2023fedcare}. This advantage can significantly benefit Radiomics, as \textit{precision medicine} \cite{chen2022radiomics} is essential for identifying patient subtypes to achieve optimal outcomes and accurately predicting prognosis \cite{bakas2020overall}. For instance, in tumor detection, patients with similar histopathological features in medical images may have varying survival probabilities \cite{hagele2020resolving}. Achieving satisfactory precision necessitates using DL over traditional methods, which require substantial computational resources (e.g., hardware accelerators \cite{nvidiaNVIDIA6000,tpu}) for training models on significant data volume, highlighting the role of Cloud computing services (e.g., Amazon AWS \cite{amazonMachineLearning} or Microsoft Azure \cite{microsoftAzureMachine}). Although such services have been utilized in healthcare systems, such as UCLA Health using Microsoft Azure to integrate and process EHR data \cite{uclahealth} and Mayo Clinic using Google AI to automate breast cancer risk scoring \cite{mayoclinic}, outsourcing sensitive data for computation to even such trusted servers poses risks. Therefore, employing methods that ensure privacy while enabling DL computation for Radiomics in potentially malicious environments is crucial.

\noindent \textbf{\em Scope of This Work:}  Utilizing DL with Radiomics (Deep Radiomics) \cite{DLforRadiomicsReview} for various purposes like detecting brain cancer \cite{DLRadiomicsBrainTumor} and gastrointestinal cancer \cite{DLforRadiomicsCancerDiag} has made a paradigm shift to replace traditional ML approaches (e.g., segmentation and feature extraction) \cite{koccak2019radiomics} for enhanced and optimized primary image processing operations. Although various Neural Networks (NNs) are employed for different EHRs (e.g., Recurrent Neural Networks (RNNs) \cite{graves2013speech} for blood pressure and EEG, and Restricted Boltzmann Machines (RBM) \cite{smolensky1986information} for image processing), this paper restricts its focus on Convolutional Neural Networks (CNNs) \cite{krizhevsky2012imagenet} as they excel in pattern recognition for medical imaging \cite{sarvamangala2022convolutional}. CNNs are specifically engineered to extract high-order hierarchical features from data through convolution operations, making them well-suited for Radiomics. Moreover, training using the Stochastic Gradient Descent (SGD) \cite{robbins1951stochastic} approach allows for rapid convergence and computational efficiency. 

To achieve privacy-preserving Deep Radiomics, this work outlines the integration of Privacy-Enhancing Technologies (PETs) \cite{PETMLSurvey,SokPPML,ppmlacmsurvey} throughout the entire Deep Radiomics pipeline, covering data collection, storage, retrieval, CNN training, and inference. These PETs encompass methods such as Searchable Encryption (SE) \cite{song2000practical}, Oblivious Random Access Machine (ORAM) \cite{goldreich1987towards}, and Private Information Retrieval (PIR) \cite{pirchor}, for private access and retrieval. Additionally, Multi-party Computation (MPC) \cite{yao1982protocols} and Homomorphic Encryption (HE) ensure secure processing under encryption, while Zero-knowledge Proof (ZKP) \cite{goldwasser2019knowledge} enables verifiable execution of Deep Radiomics. Hardware-based solutions, including Trusted Execution Environments (TEEs) \cite{intelsgx}, provide a tamper-proof computational environment within an untrusted system. Furthermore, machine learning paradigms like Federated Learning (FL) \cite{adnan2022federated} inherently preserve data privacy by keeping training data localized to each party, and Differential Privacy (DP) \cite{dwork2006differential} can contribute to privacy through statistical perturbation.



\subsection{Literature Review, Gaps and Contribution}
%%%% Generic PET surveys
%%%% SE Magazine: sewang2016secure

% Regarding private search and update, 

Several studies have focused on PETs and their broad applications, while others have specifically explored their intersections with ML. Considering the stated pipeline, notable works include \cite{sseli2023survey,sebosch2014survey}, conducting a literature review on symmetric SE and their performance and attack analysis, and \cite{pirvithana2023private} introducing PIR and its variants and extensions. Furthermore, \cite{mpc2020lindell,lindell2005secure,mpcorsini2021efficient} discussed the applications of MPC in various domains such as analytics and government collaboration and \cite{mpcdlzhou2024secure} demonstrated the integration of MPC with other PETs. Moreover, \cite{mpcdlzhang2021privacy} examined MPC techniques for DL and \cite{mpcfeng2022concretely} performed a performance analysis of private inference and training within privacy-preserving ML protocols. Studies \cite{fhemarcolla2022survey,fhemartins2017survey,wood2020homomorphic} reviewed the applications of HE in cloud computing, data aggregation, private database queries, bioinformatics, etc. \cite{fheacar2018survey} provided a theoretical review and discussed hardware implementation solutions for HE and \cite{hepodschwadt2022survey,ppdlhe,hepodschwadt2022survey} explored the use of HE in privacy-preserving DL. Regarding FE, \cite{femascia2021survey,fexu2020revisiting} outlined the functionalities of different FE schemes, describing their limitations and security models. Meanwhile, \cite{fedlpanzade2023privacy} offered a comprehensive review of the strengths and weaknesses of various approaches for FE-based PPML. ZKP for verifiable execution have been examined by \cite{zkpsun2021survey,zkpmorais2019survey}, highlighting their applications in Blockchain and Cryptocurrency transactions. \cite{zkpdlsathe2023state} analyzed ZKP for inference in PPML, comparing the performance of previous schemes, while \cite{zkpdlxing2023zero} provided a multi-layer classification of existing ZKP methods used in PPML. The constructions of TEEs have been shown by \cite{teehosam2022comprehensive}, with \cite{teevaladares2021systematic} demonstrating their applications in Cloud/Fog-Based Internet of Things (IoTs), and \cite{teedlmo2022machine,teeli2023survey} illustrating their use in ML. The role of FL has been highlighted by \cite{kaissis2020MagMedicalImage,flbanabilah2022federated,flzhang2021survey}, noting its applications in recommender systems, IoT, autonomous vehicles, and the medical sector. Lastly, DP has been investigated for statistical perturbation, with \cite{dpyang2023local} focusing on its application in statistical queries, and \cite{dpdlel2022differential} examining its usage in learning tasks along with associated challenges and solutions. Additionally, \cite{dpdlblanco2022critical} critically assessed prior applications of DP in ML, emphasizing the unsafe utilization of privacy parameters.




% Regarding Verificable exection, \cite{zkpsun2021survey} gave survey on ZKP in blockahin, \cite{zkpmohr2007survey} presented the applications of ZKP to Cryptography and \cite{zkpmorais2019survey} showed application of ZKP on cryptocurrency transactions. 

% ZKP DL (More CNN): \cite{zkpdlsathe2023state} an extensive analysis of the burgeoning field of
% Zero Knowledge Proofs within the context of machine learning applications with performance comparison of schemes in the literature and the usage of ZKP in the inference pipeline
% (**)\cite{zkpdlxing2023zero} has classified the existing
% work based concentrated on two main aspects: 1)
% the arithmetization and quantization of the machine learning
% computation process, and 2) the reduction of computational
% costs and enhancement of proving efficiency. According to
% their different focuses, the existing schemes can be can be
% classified into two main categories and three subcategories:

% \cite{fheacar2018survey} gave a pure theoretical review to hardware implementation, and \cite{fhemartins2017survey} which gave theory to motivation such as applications like private database query not how. 

% FHE DL: \cite{ppdlhe} presented the role fo a specific HE scheme in privacy-preserving DL, \cite{hepodschwadt2022survey} NNs with HE, (2) present innovative solutions and establish important techniques in the field, and (3) investigate challeng- ing problems. We discuss their pros and cons and propose some future avenues to tackle. Furthermore, we propose a set of evaluation guidelines to compare solutions in terms of resource requirements. 

% \cite{wood2020homomorphic} provides overview of fully homomorphic encryption and its applications in medicine and bioinformatics.
% \cite{mpcdlzhang2021privacy} provides data-encryption-based privacypreserving techniques with respect to (w.r.t.) linear and nonlinear computations, which are the two building blocks in DL framework. \cite{mpcfeng2022concretely} We present high-level ideas of the basic and key approaches for
% designing different styles of MPC protocols and the crucial building blocks of MPC. For MPC applications, we compare the known PPML protocols built on MPC, and describe the efficiency of private inference and training for the state-of-the-art PPML protocols.

% Regarding Verificable exection, \cite{zkpsun2021survey} gave survey on ZKP in blockahin, \cite{zkpmohr2007survey} presented the applications of ZKP to Cryptography and \cite{zkpmorais2019survey} showed application of ZKP on cryptocurrency transactions. ZKP DL (More CNN): \cite{zkpdlsathe2023state} an extensive analysis of the burgeoning field of
% Zero Knowledge Proofs within the context of machine learning applications with performance comparison of schemes in the literature and the usage of ZKP in the inference pipeline
% (**)\cite{zkpdlxing2023zero} has classified the existing
% work based concentrated on two main aspects: 1)
% the arithmetization and quantization of the machine learning
% computation process, and 2) the reduction of computational
% costs and enhancement of proving efficiency. According to
% their different focuses, the existing schemes can be can be
% classified into two main categories and three subcategories:

% Using TEEs have been shown by \cite{teevaladares2021systematic} application of TEE for Cloud/Fog-Based Internet of Things, \cite{teeli2023survey} for machine learning and encrypted database queries \cite{teehosam2022comprehensive} tee implementation using hardware and software based ones. TEE DL: \cite{teedlmo2022machine} presented the literature review of role of TEEs in confidential computing of ML with their detiald analysis of their coverage of the ML pipeline from data prepratopn to model inference. and limitations. 

% Lastly, importance of FL has been shown by \cite{flbanabilah2022federated} presented FL review with mentioning futurre applicaiotns like in recommender systems, IoT, autonomous vehicles. \cite{flzhang2021survey} FL applications in Google keyboard, medical sector, and wireless networks

% DP Surveys (***)\cite{dpyang2023local} presented two possible usage of DP one in statistical query with DP and other with Learning with DP. For each they reviewed the challenges in each direction with possible solutions to each.\cite{dpdlblanco2022critical} presented a critical review on the previous usage of DP with ML. 
% %We will show that DP-based ML implementations are mainly on the non-meaningful side. Not only because of the use of unreasonably unsafe privacy parameters, but also due to the use of relaxations that should not be counted as DP. These flaws are motivated by the attempt to salvage utility, i.e., model accuracy, which is of utmost importance in ML and is often incompatible with strict DP. In fact, in many implementations reported in the ML literature, the use of DP amounts to little more than adding noise without precise ex ante privacy guarantees. For this reason, the actual level of privacy achieved must be evaluated empirically, as typically done in the utility-first approach common in official statistics.
% \cite{dpdlel2022differential} A review of the different works based on DP for protecting users’ privacy in DL and FL. We divide these
% approaches into three categories based on their type of
% application: 1) PP queries, 2) PP datasets, 3) PP models.




%%%% Mention our focus
While there have been many solely written review papers on PETs and their broad application analysis, as described before, our scope of focus is on synergizing all the descibed PETs with the full pipeline of Deep Radiomics starting from data gathering, model training, and model inference. In the literature, there have been works that despited previous ones, have discussed a few PETs and their applications and possible hybdrid designs to ML. Examples include the introductory presentation of PETs in post-quantum era by \cite{darzi2024pqcmeetsml,ppmlpqc}, \cite{ppmlcheng} specifically delves into an ML-oriented exploration of privacy attacks, and \cite{smartppmlnpsmart} discussing encrypted computation and their hybridzation.More in-depth works include \cite{Xu2021PrivacyPreservingML,SokPPML,ppmlacmsurvey} discussing the privacy attacks against ML from ML perspective, \cite{ppdlsurvtanuwidjaja2020privacy} covering the adversarial models of MPC, HE and DP and their connection with PPDL, \cite{ppdlsurvboulemtafes2020review,ppdlmireshghallah2020privacy} categorizing the existing works in three phases of learning, inference, and model release in which the role MPC, HE, and DP have disussed in these phases, \cite{ppdlantwi2021privacy} categorizing Collaborative Deep Learning under the training stage only, and  \cite{ppdlcabrero2021sok} presented  privacy-preserving techniques for Deel learning with mainly focusing on MPC and HE and further briefly possible hybrid designs with DP and TEE, \cite{ng2023sok} offered in-depth technical analyses of previous PPDL constructions using cryptographic methods of HE and MPC and \cite{qin2023cryptographic} gave a discussion integration of PETs with ML models from SVM, different NNs.





% Surveys:
    % \cite{ppdlsurvtanuwidjaja2020privacy} Our work covers the most recent and groundbreaking methods in PPDL, specifically for MLaaS. They present the adversarial models of MPC, HE and DP and their connection with PPDL.
    % \cite{ppdlsurvboulemtafes2020review} categorized the previous works in 3 directions of learning, inference and model release and included the discussion of MPC, HE and DP (model release) as cryptographic method. in 3 levels whether distributed or individual, server-assisted or server-based.
    % \cite{ppdlmireshghallah2020privacy} looked at privacy of Deep learning in its different phases of learning, inference data aggregation (considered DP) and MPC and FHE in other phases.
    % \cite{ppdlantwi2021privacy} Keeping focus on the Collaborative/Distributed setting, we improve [10] by categorizing Collaborative Deep Learning under the training stage only and also classifying it into direct, indirect and peer-to-peer.

    % \cite{ppdlcabrero2021sok} presented  privacy-preserving techniques for Deel learning with mainly focusing on MPC and HE and further briefly possible hybrid designs with DP and TEE.
    




% magazine: ppml ppmlpqc darzi2024pqcmeetsml
%     smartppmlnpsmart kaissis2020MagMedicalImage
%     ppmlcheng: 




% Several studies in the literature address Pivacy-Preserving DL (PPDL). These studies can be categorized based on their scope as follows: The first group is \cite{ppml,ppmlpqc} that predominantly introduce identical privacy-preserving technologies and provide similar discussions without presenting distinctive advantages, except for the \cite{}, which include an additional discussion on comparing technologies and focusing on medical images, respectively. Lastly, \cite{ppmlcheng} primarily discusses privacy-preserving ML (PPML), but they are predominantly ML-oriented and lack a comprehensive discussion on all possible methods. Moreover, except \cite{ppmlcheng}, which specifically delves into an ML-oriented exploration of privacy attacks, there is a notable absence of attention to the intersection between privacy-preserving methods and ML privacy attacks in these works.  providing a comprehensive overview of the performance and system models of the PPML schemes, our contributions are outlined as follows: 


%%%% Find magazines

Despite the existance of many works in literature focusing either solely on PETs and its broad applicatios or discussing the synergizing PETs with ML, we believe, there is a gap in the literature that discusses how these PETs can benefit ML in a specific application. We outline our contribution as follows:


% \aay{1) We must first start with generic PETs surveys, stating they focus on broader PETs applications to various domains. Cite quite a bunch, and say good things about them. After state, our focus is on three aspects: (i) Healthcare and specifically radiomucs, and (ii) for it PPDL, and (iii) potential applications and hybrid approaches in mind. }

% \aay{2) PPDL works with bg surveys and magazines. Again, cite many PPDL full survey without magazine flavor, say good things about them. But state they overlap and focus on PETs aspect, and more investigation into potential of compositions might be better.}

% \aay{3) Final, I would soften the below paragraphs, and state that "They have merit of A,B, and C. Here, our goal is to do X,Y and Z, it fills the gaps in these studies, and compelemtns them blah blah. Ypu can say that we target audience of A,B and C...}

% \aay{Overall, you can create two parags (with many cites from Google Scholar on this topic) before describing contribs, or one big paragraph, explains the "scope" of this work, and then pin it down to the "use-case and composition style PETs + Radiomics literature" differentiation of ours. The most important part of the survey is to convince them that this is NEEDED, and there is not much similar of it, while acking other people and without making them angry (they are your reviewer)}. 

% \aa{Our ultimate goal is to offer a guideline for healthcare professionals, cybersecurity workforce and various domain experts on the potential application and direction of DR, who may not be an expert on PETS, advanced cryptographic or Deep Radiomics, but utilize the knowledge, taxomnomy and methods to identify the potential direction for their research and practical consideration: Something in this line, written in italic  }  


$\bullet$ {\em \ul{Providing Comprehensive Insights with Practical Aspects of PPDR}}: Recognizing the significance of Radiomics in healthcare systems, as underscored by NIH \cite{zhang2022deep}, and its integration with DL, we aim to offer unique insights into the privacy and security concerns associated with DR. Our work focuses on three key aspects: (1) It aims to balance technical details on PETs, particularly technically heavy cryptographic PETs (e.g., FHE [], MPC), while presenting their integration into DR. (2) It aims to balance the radiomics DL aspects of PETs, especially when various hybrid compositions of PETs for DR are considered. (3) It captures the main strengths and weaknesses of analyzed PETs in the context of Radiomics. Table \ref{tab:petcomp} offers detailed comparisons and insights regarding various potential compositions of PETs applied to DR. \\ \vspace{-2mm}


$\bullet$ {\em \ul{Detailed Taxonomy and Classification of Prominent PPDR with Hybrid Compositions in Mind}}:  Several PETs are available to realize PPDR with unique performance and security characteristics. We have categorized prominent PETs and security technologies into four groups based on their underlying principles when applied to DR (e.g., performance, security, architectural suitability, assumptions, etc...). Furthermore, we illustrate the potential prominent combinations of these technologies as hybrid designs. Such hybrid compositions are expected to significantly improve the practicality of PPDR over applications of PETs in isolation, often complementing their security and/or performance properties, whilst with additional costs. We outline these potential aspects visually in Figure \ref{fig:ppmlclassifcation}. \\ \vspace{-2mm}


$\bullet$ {\em \ul{Investigations on PPDR Pipelines}}: We have scrutinized the essential prerequisites of deep radiomics, offering a discussion on how each PETs can be applied across various stages of the DR and describing the pros and cons associated with each approach. This examination spans the data storage/retrieval phases and the model training and inference. Moreover, we also briefly discussed how these methods may address some of the key attacks targeting privacy in ML for radiomics. These concepts have been further visualized in Figure \ref{fig:mlpipeline}. \\ \vspace{-2mm}

\textbf{Organization - PETs Meets DR}: Figures \ref{fig:ppmlclassifcation} and Figure \ref{fig:mlpipeline} illustrate the high-level taxonomy, classification, and integration of privacy-preserving methods for Deep Radiomics, respectively. Table \ref{tab:petcomp} presents an overview of PETS for Deep Radiomics with various hybrids and their unique properties. Section 2 gives preliminaries of ML for DR. Section 3 presents our main findings and analysis on synergizing PETs and trustworthy computing with DR pipeline. Finally, the Section 4 concludes this paper. \aa{We will make this one much detailed, and move the taxo of paper info currently under main Section 3.}


$\bullet$ {\em \ul{Road map and future directions}}:


% \aay{2nd parag of Abstract in essence outlines these above three contrib bullet items, along with a short discussion of gaps before. The first parag of the abstract can be shorter. It is also useful to check the abstract word limits of our target journal, since later we may have to further shorten.}

\begin{figure*}[ht]
    \centering
    \includegraphics[width=\textwidth]{Figures/Classification.pdf}
    \caption{Taxonomy, Pros, and Cons of Essential PETs with their Prominent Hybrid Compositions for Deep Radiomics}
    \label{fig:ppmlclassifcation}
\end{figure*}





    \begin{tablenotes}
    \item[\dag] This table employs the following abbreviations: \textbf{Comp}: computation, \textbf{Comm}: communication, and \textbf{L, M, H}: Low, Mid, and High, respectively.
    
    \item[1] PET type: \textbf{C}: Cryptography-based, \textbf{H}: Hardware-based, \textbf{L}: Learning paradigm-based, \textbf{S}: Statistical-based, and \textbf{Hybrid}: Some notable hybrid designs.

    \item[2] Floating-point to fixed-point number conversion causes loss of precision and accuracy degradation.
     
    \item[3] In semi-honest security, parties execute the protocol correctly but can be curious to obtain additional information. In malicious security, parties may also deviate from the execution of the protocol. Moreover, MPC can provide $(t, n)$ threshold security where the collaboration of $t$ or more of the parties is required for the computation \cite{shamir1979share}. However, in any case, the risk of colluding servers is present.
    
    \item[4] The main properties of ZKP are Completeness, Soundness, and Zero-knowledge. (See Section \ref{sec:zkp}).
    
    \item[5] While HE and FE can be employed in training scenarios, their primary utilization focuses on the inference stage.
    
    \item[6] This is the main difference with MPC, besides the post-quantum security it provides through approaches like Lattice-based \cite{nejatollahi2019post}, Hash-based \cite{li2022hash}, etc.

    \item[7] General SE schemes leak information about files or queries to the server, including details such as the search and access patterns.

    \item[8] Obliviousness enables users to access encrypted data on an untrusted server while concealing access patterns. This can have other variants, such as distributed ORAM with threshold collusion resistance presented in \cite{hoang2017s3oram}.

    \item[9] Model size reduction can impact accuracy.

    \item[10] Setting up and managing the enclave poses overhead.


    \item[11] In FL, the training process is iteratively performed across the participating nodes and the aggregator until the model converges.

    \item[12] FL nodes engage in a multi-party computation to determine the best label for the inference output.

    \item[13] FL aggregator combines the model updates from FL nodes in each iteration, leading to a deviation from the accuracy that could be realistically attained

    \item[14] While DP is not employed individually for inference, its integration in a hybrid design with MPC and FL (See Section \ref{sec:fl}) allows for its utilization for that purpose, albeit with an augmented cost and reduced accuracy.    

    \item [15] Existence of TEE does not require full obliviousness for the search algorithm as the search and update are done in a secure enclave.
  
    \end{tablenotes}


==> notes.tex <==


research-dir FHE:
https://arxiv.org/pdf/2305.02225#page=8.15
https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=9936637#page=20.75
https://arxiv.org/pdf/2304.14397


MPC:
https://dl.acm.org/doi/pdf/10.1145/3603166.3632144#page=8.52
https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=9352960#page=13.76

FE:
https://ieeexplore.ieee.org/stamp/stamp.jsp?arnumber=10336903#page=4.71


ZKP:
https://www.politesi.polimi.it/bitstream/10589/209893/4/2023_05_Cerioli_01.pdf#page=89.23
https://arxiv.org/pdf/2310.14848#page=19.25

TEE:
https://arxiv.org/pdf/2208.10134#page=21.28

FL:
https://dl.acm.org/doi/pdf/10.1145/3501296#page=29.31
https://dl.acm.org/doi/pdf/10.1145/3412357#page=23.77

DP:
https://www.sciencedirect.com/science/article/pii/S0920548923001083#sec5
https://dl.acm.org/doi/pdf/10.1145/3436755#page=25.46



%%%%
y computation for privacy-preserving d ref errior
title of fancy boxes
